Exploring the similarity of medical imaging classification problems

Supervised learning is ubiquitous in medical image analysis. In this paper we consider the problem of meta-learning -- predicting which methods will perform well in an unseen classification problem, given previous experience with other classification problems. We investigate the first step of such an approach: how to quantify the similarity of different classification problems. We characterize datasets sampled from six classification problems by performance ranks of simple classifiers, and define the similarity by the inverse of Euclidean distance in this meta-feature space. We visualize the similarities in a 2D space, where meaningful clusters start to emerge, and show that the proposed representation can be used to classify datasets according to their origin with 89.3\% accuracy. These findings, together with the observations of recent trends in machine learning, suggest that meta-learning could be a valuable tool for the medical imaging community.

==> draft_text.tex <==
LesionCHB, LesionUNC~\cite{styner20083d} & Brain MR & 10 & 2 & 30, Classical~\cite{van2015weighting}\\


% \begin{description}
% \item[LesionCHB, LesionUNC] Segmentation of lesions in brain MR images from the MS Lesion challenge~\cite{styner20083d} (10 subjects per dataset). Each voxel is labeled as ``lesion'' or ``non-lesion'' and is described by 30 Gaussian scale space-like features~\cite{van2015weighting}
% \item[Tissue] Tissue segmentation in brain MR images (20 subjects)~\cite{Land12}. Each voxel is labeled as one of seven classes, e.g. ``white matter''~\cite{Moes16,Moes16a} and is described by 768 features, defined by the output of the fully connected layers of the convolutional neural network (CNN) in \cite{Moes16}. 
% \item[Mitosis, MitosisNorm] Mitosis detection in breast cancer histopathology images from the AMIDA13 challenge~\cite{Veta2015}. Images are used with (MitosisNorm) and without (Mitosis) prior staining normalization. Each pixel is labeled as ``mitosis'' or ``background'' and described by 200 features, defined by the output of the fully connected layer of the CNNs described in~\cite{veta2016}. 
% \item[Vessel]  Segmentation of blood vessels in retinal images from the DRIVE dataset~\todo{Reference} (20 images). Each pixel is labeled as ``vessel'' or ``background'' and described by 29 Gaussian scale space-like features~\cite{zhang2016}.
% \item[ArteryVein]  Classification of retinal vessels into arteries and veins in the DRIVE dataset. Each vessel centerline pixel is labeled as ``artery'' or ``vein'' and described by 30 features characterizing the color and color variation~\cite{dashtbozorg2014}.
% \item[Microaneurysm]  Microaneurysms detection in retinal images from the e-ophtha-MA dataset (381 images). Each candidate is labeled as ``microaneurysm'' or not, and described by 29 features, such as shape and intensity descriptors, and filter responses.
% \end{description}
%~\cite{dashtbozorg2016}->local convergence index filters

%\subsection{Representation}
%To understand the structure of the meta-representation, we would ideally like to have as many datasets as possible in the visualization. Therefore, 


%We are given labeled datasets $\{(X_i, y_i)\}_{1}^{N}$, where the $X_i$ are of any dimension, and the labels $y_i$ belong to the same label space $Y = \{1, \ldots, K\}$ \footnote{Alternatively, we could consider regression with $Y = [0,1]$ or ranking with $Y = S(\{1,\ldots,K\})$ where $S$ denotes all permutations}.

%Ideally $y_i$ reflects the best performing classifier for $X_i$, but for the purposes of this initial investigation, we label the datasets by their classification problem, i.e. $Y=$ \{tissue segmentation, \ldots \}. Our hypothesis is that datasets from the same class should form clusters in the meta-feature space, if it is chosen appropriately.    










The main problem is to define the meta-feature space. The machine learning community has focused on two possibilities: characterizing intrinsic properties of datasets, such as sample size and dimensionality, or characterizing datasets by ``landmarks'' - performances of classifiers that are easy to compute~\cite{vilalta2002perspective}. The two representations are not necessarily similar. 
Two studies on characterizing non-medical datasets~\cite{DuiPekTax2004,cheplygina2015characterizing}, show that changing dataset size and dimensionality does not always change the conclusions about how methods performed on these datasets. 


%The two representations are not necessarily similar: two studies on non-medical datasets~\cite{DuiPekTax2004,cheplygina2015characterizing}, show that changing dataset size and dimensionality does not always change the conclusions about classifier performance. 


%In doing so, we assume there is a ground-truth ``performance space'', with clusters of similar datasets.  
%In other words, the datasets became less similar in the chosen meta-feature space, but not in the performance space.
%and proposed to characterize datasets by performances of methods instead. 
%The idea is that if the datasets are similar in terms of landmark classifiers, they will also be similar in terms of more demanding classifiers.

The goal of the colleague with application D is to select the best possible method for his or her problem. 


%An advantage of MDS is that out-of-sample embedding is possible, i.e. novel datasets can be added without changing the configuration of existing samples. 



%To represent the datasets, we train the following six classifiers, mainly owing to their speed and diversity (linear vs non-linear): 
% \begin{itemize}
% \item Nearest mean classifier
% \item Linear discriminant classifier
% \item Quadratic discriminant classifier
% \item Logistic classifier 
% \item 1-nearest neighbor classifier
% \item Decision tree classifier 
% \end{itemize}

\todo{Mitko: Supervised learning is ubiquitous in medical image analysis. In this paper we consider the problem of meta-learning -- predicting which methods will perform well in a previously unseen problem, given previous experience with several classification problems. We investigate the first step of such an approach: how to quantify the similarity of different classification problems. Datasets sampled from 8 classification problems are characterized by the performance ranks of simple classifiers, and the similarity is defined by the inverse of the Euclidean distance in this meta-feature space. We visualize the similarities in a 2-dimensional space, discuss the structure that emerges, and give several directions for future research.}

. The features were defined as the output of the fully connected layers for each of the three input patches,

Here we considered both classical features from filter banks, as well as features extracted by CNNs.

%Several papers in medical imaging have directly applied features that were (pre)trained on completely different data sets, such as the ImageNet challenge, and shown that such features are potentially helpful in other classification tasks as well. 

%Pim:(Maybe we don't really want to go too much into this direction, because this opens a whole transfer learning discussion)
%Veronika: I agree, but it's good to keep it here for now, once we see which way the discussion is going :)

%However, it is questionable whether this representation would be helpful in predicting which classifier is best on a previously unseen problem. --> Discussion?
